Distributed Bayesian: a continuous Distributed Constraint Optimization Problem solver

In this work, the novel Distributed Bayesian (D-Bay) algorithm is presented for solving multi-agent problems within the continuous Distributed Constraint Optimization Problem (DCOP) framework. This framework extends the classical DCOP framework towards utility functions with continuous domains. Traditional DCOP solvers discretize the continuous domains, which increases the problem size exponentially. D-Bay overcomes this problem by utilizing Bayesian optimization for the adaptive sampling of variables to avoid discretization entirely. We theoretically show that D-Bay converges to the global optimum of the DCOP for Lipschitz continuous utility functions. The performance of the algorithm is evaluated empirically based on the sample efficiency. The proposed algorithm is compared to a centralized approach with equidistant discretization of the continuous domains for the sensor coordination problem. We find that our algorithm generates better solutions while requiring less samples.

==> sections/DPOP.tex <==
\section{Distributed Pseudo-tree Optimization Procedure (DPOP)}
\label{section:DPOP}


The DPOP algorithm \cite{Petcu2005a} solves a DCOP in three phases:
\begin{enumerate}
    \item[(2)] \emph{Bottom-up utility propagation}:
        From the leaves (nodes without children), the agents pass a utility message \utilityMessageLongDomain towards their parents.
        The message represents the projection of the (partial) global utility of the utility functions of the agents and its children with respect to all variables of the parent (and pseudo-parents).
        In words, it is a multidimensional array with one dimension for each variable within the message where every element represents an allocation of the variables, $\utilityMessage[\variableSet] = \operator(\functionSet[\variableSet])$.
        \\
        \\
        A utility message \utilityMessageIndexed is send by agent \agentIndexed to agent \agentIndexedOther based on the utility function set and utility messages received by its children.
        \\
        \\
        Messages are combined through the join operation $\utilityMessage^\agentIndex_{1,2} = \utilityMessage^\agentIndex_{1} \join \utilityMessage^\agentIndex_{2}$.
        This results in the union of the scopes, i.e.\
        $\functionScope(\utilityMessage^\agentIndex_{1,2}) = \functionScope(\utilityMessage^\agentIndex_1) \cup \functionScope(\utilityMessage^\agentIndex_2)$, and sums the value of the elements for all combinations of $\utilityMessage^\agentIndex_{1,2}[\variableSet] = \operator(\utilityMessage^\agentIndex_{1}[\variableSet], \utilityMessage^\agentIndex_{2}[\variableSet])$.
        \\
        \\
        All child messages are combined as \utilityMessageChildrenIndexedLong.
        The local message holds the utility values for the utility functions as, \utilityMessageLocalIndexedLong.
        The (pseudo-)parents message, which hold the utility values of the functions shared by the agent and its (pseudo-)parents, are combined as \utilityMessageParentsIndexedLong.
        \\
        \\
        The utility messages of the children \utilityMessageChildrenIndexed and (pseudo-)parents \utilityMessageParentsIndexed are combined with the utility message \utilityMessageAgentLocalIndexed to form the total utility message \utilityMessageAgentIndexed of agent \agentIndexed as \utilityMessageAgentLongIndexed.
        \\
        \\
        The resulting message \utilityMessageAgentIndexed is optimized over the local variables of the agent \agentIndexed.
        This operation is defined by a projection operator $\project$ and
        assigns the allocation of \variableMappingAgentIndexed that results in the maximal utility.
        The result is a message of lesser cardinality based on the number of variables in \variableMappingAgentIndexed.
        Formally, \projectionOperatorLong, and the scope \projectionOperatorScopeLong.
        \\
        \\
        For example, when $\utilityMessageAgentIndexed = \bigl[
            \begin{smallmatrix}
            4 & 5 \\
            6 & 7
            \end{smallmatrix}
            \bigr]
            $ with
            $\functionScope(\utilityMessageAgentIndexed) = \{ \variable_1, \variable_2 \}$,
            the projection is
            $\utilityMessageAgentIndexed \project \{\variable_1\} =
            \bigl[
            \begin{smallmatrix}
            6 & 7 \\
            \end{smallmatrix}
            \bigr]$ and $\allocation(\variable_1 | \variable_2) = \left\{ \{ \variable_1 = 2 | \variable_2 = 1 \}, \{ \variable_1 = 2 | \variable_2 = 2 \} \right\}$.
        \\
        \\
        After the projection, the message is sent towards to its parent,
        $\utilityMessage_i^{\Parent_i} = \utilityMessageAgentIndexed \project \variableMappingAgentIndexed$.
        After the root agent of the pseudo-tree (agent without parent) has finished this procedure, the value propagation phase is initiated.

    \item[(3)] \emph{Top-down value propagation}:
        Based on its child messages, the root agent chooses the optimal assignment of its local variables \variableMappingAgentIndexed as,
        $\allocationOptimal_\agentIndex = \argmax_{\allocation_\agentIndex}(\utilityMessageAgentIndexed[\variableMappingAgentIndexed])$.
        The allocation of these values is sent to all the children of the agent.
        Based on these values the children allocate their own variables,
        $\allocationOptimal_\agentIndexOther = \argmax_{\allocation_\agentIndexOther}(\utilityMessage^\agentIndexOther[\variableMappingAgentOtherIndexed] \perp \allocationOptimal_\agentIndex)$.
        Every agent repeats this process until the leaves of the tree are reached, completing the assignment $\allocationOptimal$ for all agents.
\end{enumerate}

==> style/commands/commands_DBay.tex <==
\newcommand{\sampleMessage}{\mathcmd{\mathfrak{S}}}
\newcommand{\sampleMessageIndexed}{\mathcmd{
  \sampleMessage_\variableIndex
}}
\newcommand{\sampleMessageIndexedOther}{\mathcmd{\sampleMessage_\agentIndexOther}}
\newcommand{\sampleMessageIndexedParent}{\mathcmd{\sampleMessage_\agentIndexParent}}




\newcommand{\sampleMessageText}{\mathcmd{\mathrm{\bf sample}}}
\newcommand{\utilityMessageText}{\mathcmd{\mathrm{\bf utility}}}
\newcommand{\sampleFinalMessageText}{\mathcmd{\mathrm{\bf final}}}

\newcommand{\sampleMessageBestIndexedParent}{\mathcmd{\hat{\sampleMessage}_\agentIndexParent}}
\newcommand{\sampleMessageBestIndexed}{\mathcmd{\hat{\sampleMessage}_\variableIndex}}
\newcommand{\sampleMessageBestRoot}{\mathcmd{\hat{\sampleMessage}_\agentIndexRoot}}
\newcommand{\sampleMessageBestParent}{\mathcmd{\hat{\sampleMessage}_\agentIndexParent}}
\newcommand{\sampleMessageBestOtherIndexed}{\mathcmd{\hat{\sampleMessage}_\variableIndexOther}}
\newcommand{\sampleMessageBestIndexedLong}{\mathcmd{
  \sampleMessageBestIndexed = \sampleMessageBestIndexedParent \cup \{ \hat{\assignment}_{\localVariablesIndexed} \}
}}
\newcommand{\sampleMessageBestIndexedLongInAlgorithm}{\mathcmd{
  \sampleMessageBestIndexed \coloneqq \sampleMessageBestIndexedParent \cup \{ \hat{\assignment}_{\localVariablesIndexed} \}
}}
\newcommand{\sampleMessageBestInitialIndexedLong}{\mathcmd{
  \sampleMessageBestIndexed = \{ \hat{\assignment}_{\localVariablesIndexed} \} \cup \sampleMessageBestParent
}}
\newcommand{\sampleMessageBestInitialRootLong}{\mathcmd{
  \sampleMessageBestRoot = \{ \hat{\assignment}_{\localVariablesRoot} \}
}}

\newcommand{\sampleMessageIndexedLong}{\mathcmd{
  \sampleMessageIndexed = \{ \assignment_{\localVariablesIndexed} \}
}}
\newcommand{\sampleMessageIndexedParentLong}{\mathcmd{
  \sampleMessageIndexedParent = \{ \assignment_{\localVariablesIndexedParent} \}
}}
\newcommand{\sampleMessageIndexedOtherLong}{\mathcmd{
  \sampleMessageIndexed = \sampleMessageIndexedParent \cup \{ \assignment_{\localVariablesIndexed} \}
}}
\newcommand{\sampleMessageIndexedOtherLongInAlgorithm}{\mathcmd{
  \sampleMessageIndexed \coloneqq \sampleMessageIndexedParent \cup \{ \assignment_{\localVariablesIndexed} \}
}}


\newcommand{\optimumMessage}{\mathcmd{\mathfrak{U}}}

\newcommand{\optimumMessageToParent}{\mathcmd{
  \optimumMessage_\agentIndex^\agentIndexParent
}}
\newcommand{\optimumMessageToParentLong}{\mathcmd{
  \optimumMessageToParent =
    \displaystyle\operator \Big( \optimumMessageLocal, \optimumMessageBestChild \Big)
}}
\newcommand{\optimumMessageToParentLongInAlgorithm}{\mathcmd{
  \optimumMessageToParent \coloneqq
    \displaystyle\operator \Big( \optimumMessageLocal, \optimumMessageBestChild \Big)
}}
\newcommand{\optimumMessageToParentLeafLong}{\mathcmd{
  \optimumMessageToParent =
    \displaystyle\min_{\assignment \in \searchSpace_{\localVariablesIndexed}}
    \displaystyle\operator_{\utilityFunctionIndexed \in \functionSetLocalCombinedIndexed} \Big( \utilityFunctionIndexed(\assignmentPartial ~|~ \sampleMessageIndexedParent) \Big)
}}

\newcommand{\optimumMessageLocal}{\mathcmd{
  \optimumMessage_\agentIndex
}}
\newcommand{\optimumMessageLocalLong}{\mathcmd{
  \optimumMessageLocal =
    \displaystyle\min_{\assignment \in \searchSpace_{\localVariablesIndexed}}
    \displaystyle\operator_{\utilityFunctionIndexed \in \functionSetLocalCombinedIndexed} \Big( \utilityFunctionIndexed(\assignmentPartial ~|~ \sampleMessageIndexedParent) \Big)
}}
\newcommand{\optimumMessageLocalLongInAlgorithm}{\mathcmd{
  \optimumMessageLocal \coloneqq
    \displaystyle\min_{\assignment \in \searchSpace_{\localVariablesIndexed}}
    \displaystyle\operator_{\utilityFunctionIndexed \in \functionSetLocalCombinedIndexed} \Big( \utilityFunctionIndexed(\assignmentPartial ~|~ \sampleMessageIndexedParent) \Big)
}}



\newcommand{\optimumMessageFromChild}{\mathcmd{
  \optimumMessage_\agentIndexChild^\agentIndex
}}

\newcommand{\optimumMessageBest}{\mathcmd{
  \hat{\optimumMessage}
}}
\newcommand{\optimumMessageBestChild}{\mathcmd{
  \optimumMessageBest_\agentIndex
}}
\newcommand{\optimumMessageIndexedChildren}{\mathcmd{
  \optimumMessageBestChild =
    \displaystyle\operator_{\agent_\agentIndexChild \in \ChildIndexed} \left( \optimumMessageFromChild \right)
}}
\newcommand{\optimumMessageIndexedChildrenInAlgorithm}{\mathcmd{
  \optimumMessageBestChild \coloneqq
    \displaystyle\operator_{\agent_\agentIndexChild \in \ChildIndexed} \left( \optimumMessageFromChild \right)
}}






\newcommand{\assignmentMessage}{\mathcmd{\mathfrak{X}}}
\newcommand{\assignmentMessageIndexed}{\mathcmd{
  \assignmentMessage_\agentIndex
}}
\newcommand{\assignmentMessageIndexedLong}{\mathcmd{
  \assignmentMessageIndexed = \{ \assignmentPartialAgentOptimal \}
}}

==> style/commands/commands_algorithm.tex <==
\newcommand{\ForEachSingleLine}[2]{\textbf{foreach } {#1} \textbf{do} {#2}}
\newcommand{\InputOutputSingleLine}[2]{\textbf{Input: } {#1} \hspace{1cm}\textbf{Output: } {#2}}
\newcommand{\IfSingleLine}[2]{\textbf{if } {#1} \textbf{then} {#2}}

==> style/commands/commands_bayesian.tex <==

\newcommand{\observationSet}{\mathcmd{\mathcal{O}}}
\newcommand{\observationSetLong}{\mathcmd{\observationSet_\numberOfObservations = \{\observation_1, \dots, \observation_\numberOfObservations \}}}

\newcommand{\observation}{\mathcmd{O}}
\newcommand{\observationLong}{\mathcmd{\observation = (\functionInput, \functionOutput)}}
\newcommand{\observationIndexed}{\mathcmd{\observation_\observationIndex}}

\newcommand{\observationLongIndexed}{\mathcmd{
  \observationIndexed = (\observationFunctionInput, \observationFunctionOutput)
}}
\newcommand{\observationLongIndexedVector}{\mathcmd{
  \observationIndexed = (\observationFunctionInputVector, \observationFunctionOutput)
}}

\newcommand{\observationOutputs}{\mathcmd{\functionOutput(\observationSet)}}
\newcommand{\observationOutputsLong}{\mathcmd{
  \observationOutputs =
  [\functionOutputBase_{1}, \dots, \functionOutputBase_\numberOfObservations]^\transpose
}}
\newcommand{\observationOutputIndexed}{\mathcmd{\functionOutputBase_{\observationIndex}}}
\newcommand{\observationOutputIndexedLong}{\mathcmd{
  \observationOutputIndexed = \utilityFunction(\observationInputIndexed)
}}

\newcommand{\observationInputs}{\mathcmd{\functionInput_{1:\numberOfObservations}}}
\newcommand{\observationInputIndexed}{\mathcmd{\functionInputBase_{\observationIndex}}}
\newcommand{\observationInputsLong}{\mathcmd{
  \observationInputs = \{ \observationFunctionInput : (\observationFunctionInput, \observationFunctionOutput) \in \observationSet \}
}}

\newcommand{\observationFunctionInput}{\mathcmd{
  \functionInputBase_\observationIndex
}}
\newcommand{\observationFunctionInputVector}{\mathcmd{
  \functionInput_\observationIndex
}}
\newcommand{\observationFunctionOutput}{\mathcmd{
  \functionOutputBase_\observationIndex
}}
\newcommand{\observationFunctionOutputVector}{\mathcmd{
  \functionOutput_\observationIndex
}}

\newcommand{\observationMaxSample}{\mathcmd{\functionOutputBase^{+}}}
\newcommand{\observationMaxSampleLong}{\mathcmd{
  \observationMaxSample = \max \{ \functionOutputBaseIndexed ~:~ (\observationFunctionInput, \observationFunctionOutput) \in \observationSet \}
}}

\newcommand{\observationMaxSampleInput}{\mathcmd{\functionInputBase^{+}}}
\newcommand{\observationMaxSampleInputLong}{\mathcmd{
  \observationMaxSampleInput =
  \{ \observationFunctionInput ~:~ (\observationFunctionInput, \observationFunctionOutput) \in \observationSet ~|~ \observationFunctionOutput = \observationMaxSample \}
}}

\newcommand{\kernel}{\mathcmd{\kappa}}
\newcommand{\kernelBold}{\mathcmd{\bm{\kappa}}}
\newcommand{\kernelDot}{\mathcmd{\kernel(\cdot, \cdot)}}
\newcommand{\kernelX}{\mathcmd{\kernel(\functionInputBase, \functionInputBase)}}
\newcommand{\kernelIndexed}{\mathcmd{
  \kernel(\functionInputBaseIndexed, \functionInputBaseIndexedOther)
}}
\newcommand{\kernelLong}{\mathcmd{
  \kernel(\functionInputBase, \functionInputBase^\prime) =
  \expectation \left[
    \big( \utilityFunction(\functionInputBase) - \gpMeanFunction(\functionInputBase) \big)
    \big( \utilityFunction(\functionInputBase^\prime) - \gpMeanFunction(\functionInputBase^\prime) \big)^\transpose
  \right]
}}

\newcommand{\kernelCrossCorrelation}{\mathcmd{\bm{k}(\functionInputBase | \observationSet)}}
\newcommand{\kernelCrossCorrelationLong}{\mathcmd{
  \kernelCrossCorrelation = [\kernel\bracket{\functionInputBase_{1}, \functionInputBase}, \dots, \kernel\bracket{\functionInputBase_\numberOfObservations, \functionInputBase}]^\transpose
}}

\newcommand{\kernelGramianBase}{\mathcmd{K}}
\newcommand{\kernelGramian}{\mathcmd{\bm{K}}}
\newcommand{\kernelGramianLong}{\mathcmd{
  (\kernelGramian)_{\variableIndex, \variableIndexOther} = \kernelIndexed \text{ for all } \variableIndex, \variableIndexOther \in \{1,\dots,\numberOfObservations\}
}}

\newcommand{\kernelScale}{\mathcmd{\lambda}}
\newcommand{\kernelLength}{\mathcmd{l}}
\newcommand{\kernelHyper}{\mathcmd{\nu}}

\newcommand{\kernelHelperZ}{\mathcmd{z}}
\newcommand{\kernelHelperZLong}{\mathcmd{
  \kernelHelperZ = \frac{\sqrt{3} \| \functionInputBase_2 - \functionInputBase_1 \|}{\kernelLength}
}}

\newcommand{\kernelHelperZOne}{\mathcmd{\kernelHelperZ_1}}
\newcommand{\kernelHelperZOneLong}{\mathcmd{
  \kernelHelperZOne = \frac{\sqrt{3} \| \functionInput_1 - \functionInput \|}{\kernelLength}
}}

\newcommand{\kernelHelperZTwo}{\mathcmd{\kernelHelperZ_2}}
\newcommand{\kernelHelperZTwoLong}{\mathcmd{
  \kernelHelperZTwo = \frac{\sqrt{3} \| \functionInput_2 - \functionInput \|}{\kernelLength}
}}

\newcommand{\kernelHelperOne}{\mathcmd{\kernel_1}}
\newcommand{\kernelHelperOneLong}{\mathcmd{
  \kernelHelperOne = \kernelScale^2 ( 1 + \kernelHelperZOne ) e^{-\kernelHelperZOne}
}}

\newcommand{\kernelHelperTwo}{\mathcmd{\kernel_2}}
\newcommand{\kernelHelperTwoLong}{\mathcmd{
  \kernelHelperTwo = \kernelScale^2 ( 1 + \kernelHelperZTwo ) e^{-\kernelHelperZTwo}
}}

\newcommand{\kernelHelperOneTwo}{\mathcmd{\kernel_{12}}}
\newcommand{\kernelHelperTwoOne}{\mathcmd{\kernel_{21}}}
\newcommand{\kernelHelperOneTwoLong}{\mathcmd{
  \kernelHelperOneTwo = \kernelHelperTwoOne = \kernelScale^2 ( 1 + \kernelHelperZ ) e^{-\kernelHelperZ}
}}

\newcommand{\kernelObservationMidPoint}{\mathcmd{\functionInputBase_d}}
\newcommand{\kernelObservationMidPointLong}{\mathcmd{
  \kernelObservationMidPoint = \frac{1}{2}(\functionInputBase_2 - \functionInputBase_1)
}}



\newcommand{\deviationFunctionBase}{\mathcmd{\sigma}}
\newcommand{\deviationFunction}{\mathcmd{\deviationFunctionBase(\functionInputBase | \observationSet)}}
\newcommand{\deviationFunctionVector}{\mathcmd{\deviationFunctionBase(\functionInput | \observationSet)}}
\newcommand{\deviationFunctionDot}{\mathcmd{\deviationFunctionBase(\cdot | \observationSet)}}

\newcommand{\varianceFunctionBase}{\mathcmd{\deviationFunctionBase^2}}
\newcommand{\varianceFunctionObservations}{\mathcmd{
  \varianceFunctionBase(\functionInput | \observation_{1:2})
}}
\newcommand{\deviationFunctionObservationsMidPoint}{\mathcmd{
  \deviationFunctionBase(\kernelObservationMidPoint | \observation_{1:2})
}}
\newcommand{\varianceFunctionObservationsMidPoint}{\mathcmd{
  \varianceFunctionBase(\kernelObservationMidPoint | \observation_{1:2})
}}
\newcommand{\varianceFunctionObservationsMidPointExpended}{\mathcmd{
  \kernelScale^2 \left( 1 - \frac{2 k_d^2 }{1 + k_{z}} \right)
}}
\newcommand{\varianceFunctionObservationsMidPointLong}{\mathcmd{
  \varianceFunctionObservationsMidPoint &= \varianceFunctionObservationsMidPointExpended
}}

\newcommand{\varianceFunction}{\mathcmd{\varianceFunctionBase(\functionInputBase | \observationSet)}}
\newcommand{\varianceFunctionDot}{\mathcmd{\varianceFunctionBase(\cdot | \observationSet)}}

\newcommand{\varianceFunctionVector}{\mathcmd{\varianceFunctionBase(\functionInput | \observationSet)}}


\newcommand{\varianceFunctionExtended}{\mathcmd{
  \kernelX - \kernelCrossCorrelation^\transpose \kernelGramian^{-1} (\observationSet)\kernelCrossCorrelation
}}
\newcommand{\varianceFunctionLong}{\mathcmd{
  \varianceFunction = \varianceFunctionExtended
}}


\newcommand{\meanFunctionBase}{\mathcmd{\mu}}
\newcommand{\meanFunction}{\mathcmd{
  \meanFunctionBase(\functionInputBase | \observationSet)
}}
\newcommand{\meanFunctionDot}{\mathcmd{
  \meanFunctionBase(\cdot | \observationSet)
}}
\newcommand{\meanFunctionVector}{\mathcmd{
  \meanFunctionBase(\functionInput | \observationSet)
}}
\newcommand{\meanFunctionMidPoint}{\mathcmd{
  \meanFunctionBase(\kernelObservationMidPoint | \observationSet_{1:2})
}}
\newcommand{\meanFunctionExtended}{\mathcmd{
  \kernelCrossCorrelation^\transpose \kernelGramian^{-1}(\observationSet) \observationOutputs
}}
\newcommand{\meanFunctionLong}{\mathcmd{
  \meanFunction = \meanFunctionExtended
}}

\newcommand{\meanFunctionDerivative}{\mathcmd{
  \frac{\mathrm{d} \meanFunctionBase(\functionInput | \observationSet_{1:2})}{\mathrm{d} \functionInput}
}}
\newcommand{\meanFunctionDerivativeLong}{\mathcmd{
  \meanFunctionDerivative =
  -\frac{\kernelScale^2 \sqrt{3} }{\kernelLength} \Big( \kernelHelperZOne \mathrm{e}^{-\kernelHelperZOne} \kernelGramianBase_1 - \kernelHelperZTwo \mathrm{e}^{-\kernelHelperZTwo} \kernelGramianBase_2 \Big)
}}

\newcommand{\meanFunctionDerivativeRatio}{\mathcmd{
  \frac{\| \functionInput_2 - \functionInput_1 \|}{\kernelLength}
}}

\newcommand{\meanFunctionDerivativeSingle}{\mathcmd{
  \frac{\mathrm{d} \meanFunctionBase(\functionInputBase | \observation_1)}{\mathrm{d} \functionInputBase}
}}
\newcommand{\meanFunctionDerivativeSingleLong}{\mathcmd{
  \meanFunctionDerivativeSingle =
  -3 \functionOutput_1
  \frac{ ( \functionInput - \functionInput_1 ) }{ \kernelLength }
  \mathrm{exp}\bracket{
    \frac{-\sqrt{3}}{\kernelLength} \| \functionInput - \functionInput_1 \|
  }
}}

\newcommand{\meanFunctionDerivativeKernelLengthSingle}{\mathcmd{
  \kernelLength \geq \frac{\sqrt{3} \mathrm{e}^{-1} \functionOutputBase_1}{ \lipschitzConstantIndexed }
}}
\newcommand{\meanFunctionDerivativeKernelLengthDouble}{\mathcmd{
  \kernelLength \geq \frac{\sqrt{3} \mathrm{e}^{-1} \upperBoundFunctionMaxOutput_{1:2} }{ \lipschitzConstantIndexed }
}}


\newcommand{\acquisitionFunctionParameter}{\mathcmd{\xi}}

\newcommand{\acquisitionFunctionBase}{\mathcmd{q}}
\newcommand{\acquisitionFunctionDot}{\mathcmd{\acquisitionFunctionBase(\cdot)}}
\newcommand{\acquisitionFunction}{\mathcmd{
  \acquisitionFunctionBase_{\mathrm{EI}}(\functionInputBase, \acquisitionFunctionParameter | \observationSet)
}}
\newcommand{\acquisitionFunctionEI}{\mathcmd{
  \acquisitionFunctionBase_{\mathrm{EI}}
}}
\newcommand{\acquisitionFunctionEIDot}{\mathcmd{
  \acquisitionFunctionEI(\cdot, \acquisitionFunctionParameter | \observationSet)
}}
\newcommand{\acquisitionFunctionVector}{\mathcmd{
  \acquisitionFunctionBase(\functionInput, \acquisitionFunctionParameter | \observationSet)
}}
\newcommand{\acquisitionFunctionNoParameter}{\mathcmd{
  \acquisitionFunctionBase(\functionInputBase, 0 | \observationSet)
}}

\newcommand{\acquisitionExpectedImprovementExtended}{\mathcmd{
  \expectation \Big[ \big(\utilityFunction(\functionInput) \geq (\observationMaxSample + \acquisitionFunctionParameter) \big)_{+} \Big]
}}
\newcommand{\acquisitionExpectedImprovementLong}{\mathcmd{
  \acquisitionFunction = \acquisitionExpectedImprovementExtended
}}

\newcommand{\acquisitionFunctionLong}{\mathcmd{
  \acquisitionFunction =
  \begin{cases}
    \acquisitionFunctionNonZeroLong &\text{if } \deviationFunction > 0\\
    0 &\text{if } \deviationFunction = 0
  \end{cases}
}}
\newcommand{\acquisitionFunctionNonZeroCumulativeLong}{\mathcmd{
  \acquisitionHelper \Phi\bracket{ \frac{\acquisitionHelper}{\deviationFunction} }
}}
\newcommand{\acquisitionFunctionNonZeroDensityLong}{\mathcmd{
  \deviationFunction \phi\bracket{ \frac{\acquisitionHelper}{\deviationFunction} }
}}
\newcommand{\acquisitionFunctionNonZeroLong}{\mathcmd{
  \acquisitionFunctionNonZeroCumulativeLong + \acquisitionFunctionNonZeroDensityLong
}}


\newcommand{\acquisitionHelper}{\mathcmd{
  z(\functionInputBase, \acquisitionFunctionParameter | \observationSet)
}}
\newcommand{\acquisitionHelperNoParameterLong}{\mathcmd{
  \meanFunction - \observationMaxSample
}}
\newcommand{\acquisitionHelperExtended}{\mathcmd{
  \meanFunction - \left(\observationMaxSample + \acquisitionFunctionParameter\right)
}}
\newcommand{\acquisitionHelperExtendedNoParameter}{\mathcmd{
  \meanFunction - \observationMaxSample
}}
\newcommand{\acquisitionHelperLong}{\mathcmd{
  \acquisitionHelper = \acquisitionHelperExtended
}}



\newcommand{\nextSample}{\mathcmd{\observationInputIndexed}}
\newcommand{\nextSampleLong}{\mathcmd{\observationFunctionInput = \argmax_{\functionInput} \acquisitionFunction}}



\newcommand{\searchRegion}{\mathcmd{\mathcal{S}}}
\newcommand{\searchRegionLong}{\mathcmd{\searchRegion = \{ \functionInputBase \in \domainOperator(\utilityFunction) ~:~ \acquisitionFunctionBase(\functionInputBase, \acquisitionFunctionParameter | \observationSet) > 0 \}}}

\newcommand{\upperBoundRegion}{\mathcmd{\mathcal{U}}}
\newcommand{\upperBoundRegionLong}{\mathcmd{\upperBoundRegion = \{ \functionInputBase \in \domainOperator(\utilityFunction) ~:~ \upperBoundFunction > \observationMaxSample \} }}
\newcommand{\upperBoundRegionLongIndexed}{\mathcmd{\upperBoundRegion_\functionIndex = \{ \functionInputIndexed ~:~ \upperBoundFunctionIndexed > \observationMaxSample_\functionIndex \} }}


\newcommand{\upperBoundFunctionBase}{\mathcmd{
  \bar{\utilityFunction}
}}
\newcommand{\upperBoundFunction}{\mathcmd{
  \upperBoundFunctionBase(\functionInputBase | \observationSet)
}}
\newcommand{\upperBoundFunctionDot}{\mathcmd{
  \upperBoundFunctionBase(\cdot)
}}
\newcommand{\upperBoundFunctionMidPoint}{\mathcmd{
  \upperBoundFunctionBase(\kernelObservationMidPoint | \observationSet_{1:2})
}}

\newcommand{\upperBoundFunctionIndexed}{\mathcmd{
  \bar{\utilityFunctionIndexed}(\functionInput | \observationSet)
}}
\newcommand{\upperBoundFunctionLongIndex}{\mathcmd{
  \upperBoundFunction = \min \{ \lipschitzConstantIndexed | \functionInputBase - \observationFunctionInput | + \observationFunctionOutput ~:~ (\observationFunctionInput, \observationFunctionOutput) \in \observationSet \}
}}
\newcommand{\upperBoundFunctionMaxInput}{\mathcmd{\bar{\functionInputBase}}}
\newcommand{\upperBoundFunctionMaxInputLong}{\mathcmd{
  \upperBoundFunctionMaxInput =
  \underaccent{\functionInputBase \in \domainOperator(\utilityFunction)}{\argmax}
  \upperBoundFunction
}}

\newcommand{\upperBoundFunctionMaxOutput}{\mathcmd{\bar{\functionOutputBase}}}
\newcommand{\upperBoundFunctionMaxOutputLong}{\mathcmd{
  \upperBoundFunctionMaxOutput =
  \underaccent{\functionInputBase \in \domainOperator(\utilityFunction)}{\max}
  \upperBoundFunction
}}

\newcommand{\lowerBoundFunctionBase}{\mathcmd{
  \munderbar{\utilityFunction}
}}
\newcommand{\lowerBoundFunction}{\mathcmd{
  \lowerBoundFunctionBase(\functionInputBase | \observationSet)
}}
\newcommand{\lowerBoundFunctionObservation}{\mathcmd{
  \lowerBoundFunctionBase(\functionInputBase_\observationIndex | \observationSet)
}}
\newcommand{\lowerBoundFunctionLongIndex}{\mathcmd{
  \lowerBoundFunction = \max \{ -\lipschitzConstantIndexed | \functionInputBase - \observationFunctionInput | + \observationFunctionOutput ~:~ (\observationFunctionInput, \observationFunctionOutput) \in \observationSet \}
}}

\newcommand{\functionInputOptimal}{\mathcmd{\functionInputBase^*}}
\newcommand{\functionInputOptimalLong}{\mathcmd{
    \functionInputOptimal =
    \argmax_{\functionInputBase \in \searchSpaceFunctionIndexed}
    \utilityFunctionIndexed(\functionInputBase)
}}
\newcommand{\functionInputOptimalLongIndexed}{\mathcmd{
    \functionInputOptimal_\functionIndex =
    \argmax_{\observationFunctionInput}
    \utilityFunctionIndexed
}}

\newcommand{\functionOutputOptimal}{\mathcmd{\functionOutputBase^*}}
\newcommand{\functionOutputOptimalLong}{\mathcmd{
    \functionOutputOptimal =
    \max_{\functionInputBase \in \searchSpaceFunctionIndexed}
    \utilityFunctionIndexed(\functionInputBase)
    }}
\newcommand{\functionOutputOptimalLongIndexed}{\mathcmd{
    \functionOutputOptimal_\functionIndex = \max_{\observationFunctionInput} \utilityFunctionIndexed
}}

\newcommand{\lipschitzConstant}{\mathcmd{L}}
\newcommand{\lipschitzConstantIndexed}{\mathcmd{
  \lipschitzConstant_\utilityFunction
}}
\newcommand{\lipschitzConstantIndexedLong}{\mathcmd{
  | \utilityFunction(\functionInputBaseIndexed) - \utilityFunction(\functionInputBaseIndexedOther) | \leq \lipschitzConstantIndexed | \functionInputBaseIndexed - \functionInputBaseIndexedOther |
}}
\newcommand{\lipschitzFunction}{\mathcmd{l}}
\newcommand{\lipschitzFunctionIndexed}{\mathcmd{
  \lipschitzFunction_{\utilityFunction, \observationIndex}(\functionInput | \observationIndexed)
}}


\newcommand{\functionInputBase}{\mathcmd{x}}
\newcommand{\functionInputBaseIndexed}{\mathcmd{\functionInputBase_\variableIndex}}
\newcommand{\functionInputBaseIndexedOther}{\mathcmd{\functionInputBase_\variableIndexOther}}

\newcommand{\functionInput}{\mathcmd{\bm{x}}}
\newcommand{\functionInputIndexed}{\mathcmd{\functionInput_\variableIndex}}
\newcommand{\functionInputIndexedOther}{\mathcmd{\functionInput_\variableIndexOther}}

\newcommand{\functionOutputBase}{\mathcmd{y}}
\newcommand{\functionOutputBaseIndexed}{\mathcmd{\functionOutputBase_\observationIndex}}

\newcommand{\functionOutput}{\mathcmd{\bm{y}}}
\newcommand{\functionOutputIndexed}{\mathcmd{\functionOutput_\observationIndex}}
\newcommand{\functionOutputLongIndexed}{\mathcmd{
  \observationFunctionOutput = \utilityFunction(\observationFunctionInput)
}}
\newcommand{\functionOutputLongIndexedVector}{\mathcmd{
  \observationFunctionOutput = \utilityFunction(\observationFunctionInputVector)
}}

\newcommand{\regret}{\mathcmd{r}}
\newcommand{\regretLong}{\mathcmd{
    \regret = | \upperBoundFunctionMaxOutput - \observationMaxSample |
}}
\newcommand{\regretMax}{\mathcmd{\bar{\regret}}}

\newcommand{\regretMaxDistance}{\mathcmd{\functionInputBase_\regret}}
\newcommand{\regretMaxDistanceLong}{\mathcmd{
  \regretMaxDistance = \frac{\regretMax}{\lipschitzConstantIndexed}
}}

\newcommand{\regretMaxHelper}{\mathcmd{z_\regret}}
\newcommand{\regretMaxHelperLong}{\mathcmd{
  \regretMaxHelper = \frac{\sqrt{3}}{\kernelLength} \regretMaxDistance
}}

\newcommand{\regretMaxHelperK}{\mathcmd{k_\regret}}
\newcommand{\regretMaxHelperKLong}{\mathcmd{
  \regretMaxHelperK = (1 + \frac{1}{2}\regretMaxHelper) \mathrm{e}^{-\frac{1}{2}\regretMaxHelper}
}}

\newcommand{\regretMaxHelperKTwo}{\mathcmd{k_{2\regret}}}
\newcommand{\regretMaxHelperKTwoLong}{\mathcmd{
  \regretMaxHelperKTwo = (1 + \regretMaxHelper) \mathrm{e}^{-\regretMaxHelper}
}}

\newcommand{\gp}{\mathcmd{\mathrm{GP}}}
\newcommand{\NormalDistribution}{\mathcmd{\mathcal{N}}}

\newcommand{\gpMeanFunction}{\mathcmd{m}}
\newcommand{\gpMeanFunctionIndexed}{\gpMeanFunction_\functionIndex}
\newcommand{\gpMeanFunctionIndexedOther}{\gpMeanFunction_\functionIndexOther}
\newcommand{\gpMeanFunctionDot}{\mathcmd{\gpMeanFunction(\cdot)}}
\newcommand{\gpMeanFunctionLong}{\mathcmd{
  \gpMeanFunction(\functionInputBase) = \expectation\left[ \utilityFunction(\functionInputBase) \right]
}}

\newcommand{\probability}{\mathcmd{P}}
\newcommand{\expectation}{\mathcmd{\mathds{E}}}

\newcommand{\maternKernel}{\mathcmd{\kernel_{\mathrm{Mat}}}}
\newcommand{\maternKernelLong}{\mathcmd{
  \maternKernel(\functionInputIndexed, \functionInputIndexedOther) &=
    \kernelScale^2 \bracket{
        1 + \frac{\sqrt{3}\|\functionInputIndexed, \functionInputIndexedOther\|}{\kernelLength}
    }
    \mathrm{exp} \bracket{
        -\frac{\sqrt{3}\|\functionInputIndexed, \functionInputIndexedOther\|}{\kernelLength}
    }
}}

\newcommand{\dirichletKernel}{\mathcmd{\kernel_{\mathrm{d}}}}
\newcommand{\dirichletKernelLong}{\mathcmd{
  \dirichletKernel(\functionInputBaseIndexed, \functionInputBaseIndexedOther) = \kernelScale^2 \min(\functionInputBaseIndexed, \functionInputBaseIndexedOther) (1 - \max(\functionInputBaseIndexed, \functionInputBaseIndexedOther))
}}


==> style/commands/commands_dcop.tex <==
\newcommand{\DCOPTuple}{\mathcmd{\mathfrak{D}}}
\newcommand{\DCOPTupleLong}{\mathcmd{\DCOPTuple = \langle\agentSet, \variableSet, \domainSet, \functionSet, \variableMapping, \operator\rangle}}

\newcommand{\globalUtility}{\mathcmd{G}}
\newcommand{\globalUtilityLong}{\mathcmd{
  \globalUtility(\assignment) = \underaccent{\utilityFunctionIndexed \in \functionSet}{\operator}~
  \Big(
    \utilityFunctionIndexed(\assignmentPartial)
  \Big)
}}

\newcommand{\variableMapping}{\mathcmd{\alpha}}
\newcommand{\variableMappingLong}{\mathcmd{\variableMapping :~ \variableSet \rightarrow \agentSet}}

\newcommand{\variableMappingAgentIndexed}{\mathcmd{
  \variableMapping(\variableIndexed)
}}
\newcommand{\variableMappingAgentOtherIndexed}{\mathcmd{
  \variableMapping(\variableIndexedOther)
}}

\newcommand{\localVariables}{\mathcmd{\variableSet}}
\newcommand{\localVariablesIndexed}{\mathcmd{
  \localVariables_{\variableIndex}
}}
\newcommand{\localVariablesRoot}{\mathcmd{
  \localVariables_{\agentIndexRoot}
}}
\newcommand{\localVariablesOtherIndexed}{\mathcmd{\localVariables_{\variableIndexOther}}}
\newcommand{\localVariablesIndexedOther}{\mathcmd{\localVariables_{\variableIndexOther}}}
\newcommand{\localVariablesIndexedParent}{\mathcmd{\localVariables_{\agentIndexParent}}}

\newcommand{\localVariablesIndexedLong}{\mathcmd{
  \localVariablesIndexed = \{ \variableIndexedOther \in \variableSet ~|~ \agentIndexed \in \variableMappingAgentOtherIndexed\}
}}

\newcommand{\operatorLong}{\mathcmd{\operator ~:~ \functionSet \rightarrow \realsSet }}

\newcommand{\searchSpace}{\mathcmd{\mathbf{\Sigma}}}
\newcommand{\searchSpaceLong}{\mathcmd{
  \searchSpace = \prod_{\variableIndex = 1}^{\numberOfVariables} \domainSetIndexed
}}
\newcommand{\searchSpaceAll}{\mathcmd{\searchSpace_\variableSet}}

\newcommand{\searchSpaceFunctionIndexed}{\mathcmd{\searchSpace_{\variableSetFunctionIndexed}}}


\newcommand{\assignment}{\mathcmd{\sigma}}
\newcommand{\assignmentCompleteLong}{\mathcmd{
  \assignment : \variableSet \rightarrow \searchSpace
  }}
\newcommand{\assignmentComplete}{\mathcmd{\assignment_{\variableSet}}}

\newcommand{\assignmentPartialBase}{\mathcmd{
  \assignment_\variableSetFunction
}}

\newcommand{\assignmentIndexed}{\mathcmd{
  \assignment(\variableIndexed)
}}

\newcommand{\assignmentSingleLong}{\mathcmd{
  \assignmentIndexed : \variableIndexed \rightarrow \domainSetIndexed
}}

\newcommand{\assignmentPartialLong}{\mathcmd{
  \assignmentPartialBase = \{ \assignmentIndexed ~:~ \variableIndexed \in \variableSetFunction \}
}}

\newcommand{\assignmentPartial}{\mathcmd{
  \assignment_{\variableSetFunctionIndexed}
}}

\newcommand{\assignmentPartialOptimal}{\mathcmd{
  \hat{\assignment}
}}


\newcommand{\assignmentPartialAgentOptimal}{\mathcmd{
  \hat{\assignment}_{\localVariablesIndexed}
}}
\newcommand{\assignmentPartialAgentOtherOptimal}{\mathcmd{
  \hat{\assignment}_{\localVariablesOtherIndexed}
}}

\newcommand{\assignmentPartialAgentGlobalOptimal}{\mathcmd{
  \assignment^*_{\localVariablesIndexed}
}}

\newcommand{\assignmentPartialAgentOptimalLong}{\mathcmd{
  \assignmentPartialAgentOptimal =
  \underaccent{\assignment \in \searchSpace_{\localVariablesIndexed}}{\argmax}~~~~~~~~
    \underaccent{\utilityFunctionIndexed \in \functionSetLocalIndexed \cup \functionSetSharedIndexed}{\operator} \left( \utilityFunctionIndexed(\assignmentPartial) \right)
}}


\newcommand{\assignmentOptimal}{\mathcmd{\assignment^*}}
\newcommand{\assignmentOptimalLong}{\mathcmd{
  \assignmentOptimal \coloneqq \underaccent{\assignment \in \searchSpace}{\argmax} \globalUtility(\assignment)
}}


\newcommand{\allocation}{\mathcmd{\mathfrak{X}}}
\newcommand{\allocationIndexedLong}{\mathcmd{
  \allocation(\variableSet) = \{\allocationOperator(\variableIndexed) ~:~ \variableIndexed \in \variableSet \}
}}

\newcommand{\allocationVariable}{\mathcmd{\mathfrak{x}}}

\newcommand{\allocationOperatorLong}{\mathcmd{\allocationOperator ~:~ \variableSet \rightarrow (\domainSet \in \domainSet)}}

\newcommand{\allocationOptimal}{\mathcmd{\allocation^*}}

\newcommand{\projectionLong}{\mathcmd{\utilityFunction[\variableSet] = \utilityFunction(\allocation(\variableSet))}}

\newcommand{\projectionOperatorLong}{\mathcmd{\utilityMessageAgentIndexed \perp \variableMappingAgentIndexed = \max_{\variableMappingAgentIndexed} \utilityMessageAgentIndexed[\variableMappingAgentIndexed]}}
\newcommand{\projectionOperatorScopeLong}{\mathcmd{\functionScope(\utilityMessageAgentIndexed \perp \variableMappingAgentIndexed) = \functionScope(\utilityMessageAgentIndexed) \setminus \variableMappingAgentIndexed}}


\newcommand{\agent}{\mathcmd{a}}
\newcommand{\agentIndexed}{\mathcmd{\agent_\agentIndex}}
\newcommand{\agentIndexedOther}{\mathcmd{\agent_\agentIndexOther}}

\newcommand{\agentIndexedParent}{\mathcmd{\agent_\agentIndexParent}}
\newcommand{\agentIndexedChild}{\mathcmd{\agent_\agentIndexChild}}

\newcommand{\agentSet}{\mathcmd{\mathbf{A}}}
\newcommand{\agentSetLong}{\mathcmd{\agentSet = \{ \agent_\agentIndexRoot, \dots, \agent_\numberOfAgents \}}}

\newcommand{\variable}{\mathcmd{x}}
\newcommand{\variableIndexed}{\mathcmd{\variable_\variableIndex}}
\newcommand{\variableIndexedOther}{\mathcmd{\variable_\variableIndexOther}}

\newcommand{\variableSetIndexed}{\mathcmd{\mathbf{\variable}^\variableIndex}}

\newcommand{\variableSetFunction}{\mathcmd{\mathbf{V}}}
\newcommand{\variableSetFunctionIndexed}{\mathcmd{
  \variableSetFunction_\functionIndex
}}
\newcommand{\variableSetFunctionIndexedLong}{\mathcmd{
  \variableSetFunctionIndexed \subseteq \variableSet
}}

\newcommand{\variableSetOtherIndexed}{\mathcmd{\variableSet_\agentIndexOther}}

\newcommand{\variableSet}{\mathcmd{\mathbf{X}}}
\newcommand{\variableSetLong}{\mathcmd{
  \variableSet = \{ \variable_\agentIndexRoot, \dots, \variable_\numberOfVariables \}
}}

\newcommand{\variableSetParentIndexed}{\mathcmd{\variableMapping(\ParentIndexed)}}
\newcommand{\variableSetPseudoParentIndexed}{\mathcmd{\variableMapping(\PseudoParentIndexed)}}


\newcommand{\domain}{\mathcmd{d}}


\newcommand{\domainSet}{\mathcmd{\mathbf{D}}}
\newcommand{\domainSetIndexed}{\mathcmd{\domainSet_\variableIndex}}
\newcommand{\domainSetLong}{\mathcmd{\domainSet = \{ \domainSet_\agentIndexRoot, \dots, \domainSet_\numberOfVariables \}}}

\newcommand{\utilityFunction}{\mathcmd{f}}
\newcommand{\utilityFunctionDot}{\mathcmd{\utilityFunction(\cdot)}}
\newcommand{\utilityFunctionIndexed}{\mathcmd{\utilityFunction_\functionIndex}}
\newcommand{\utilityFunctionIndexedDot}{\mathcmd{\utilityFunctionIndexed(\cdot)}}

\newcommand{\functionSet}{\mathcmd{\mathbf{F}}}
\newcommand{\functionSetLong}{\mathcmd{\functionSet = \{ \utilityFunction_\agentIndexRoot, \dots, \utilityFunction_\numberOfFunctions \}}}

\newcommand{\functionSetLocalIndexed}{\mathcmd{
  \functionSet_{\agentIndexed}
}}
\newcommand{\functionSetLocalOtherIndexed}{\mathcmd{
  \functionSet_{\variableIndexOther}
}}
\newcommand{\functionSetLocalLongIndexed}{\mathcmd{
  \functionSetLocalIndexed = \{
    \utilityFunctionIndexed \in \functionSet :
       \functionScopeIndexed = \{\agentIndexed\}
  \}
}}

\newcommand{\functionSetLocalCombinedIndexed}{\mathcmd{
  \functionSet_{\variableIndex}
}}
\newcommand{\functionSetLocalCombinedRoot}{\mathcmd{
  \functionSet_{\agentIndexRoot}
}}
\newcommand{\functionSetLocalCombinedIndexedLong}{\mathcmd{
  \functionSetLocalCombinedIndexed = \functionSetLocalIndexed \cup \functionSetSharedIndexed
}}
\newcommand{\functionSetLocalCombinedChild}{\mathcmd{
  \functionSet_{\agentIndexChild}
}}



\newcommand{\functionSetSharedIndexed}{\mathcmd{
  \functionSet_{\Parent, \variableIndex}
}}
\newcommand{\functionSetSharedIndexedOther}{\mathcmd{
  \functionSet_{\Parent, \variableIndexOther}
}}
\newcommand{\functionSetSharedLongIndexed}{\mathcmd{
  \functionSetSharedIndexed = \{
    \utilityFunctionIndexed \in \functionSet :
    \left(\agentIndexed \in \functionScopeIndexed\right)
    \land
    \left(\functionScopeIndexed \cap (\ParentIndexed \cup \PseudoParentIndexed) \neq \emptyset\right)
  \}
}}

\newcommand{\functionScope}{\mathcmd{\variableMapping}}
\newcommand{\functionScopeIndexed}{\mathcmd{\functionScope(\variableSetFunctionIndexed)}}
\newcommand{\functionScopeLongIndexed}{\mathcmd{
  \functionScopeIndexed = \{ \functionScope(\variable) \in \agentSet ~|~ \variable \in \variableSetFunctionIndexed \}
}}

==> style/commands/commands_dfs.tex <==
\newcommand{\Parent}{\mathcmd{\mathrm{\bf{P}}}}
\newcommand{\ParentIndexed}{\mathcmd{\Parent_{\variableIndex}}}
\newcommand{\ParentIndexedOther}{\mathcmd{\Parent_{\variableIndexOther}}}

\newcommand{\PseudoParent}{\mathcmd{\mathrm{\bf{PP}}}}
\newcommand{\PseudoParentIndexed}{\mathcmd{\PseudoParent_{\variableIndex}}}

\newcommand{\Child}{\mathcmd{\mathrm{\bf{C}}}}
\newcommand{\ChildIndexed}{\mathcmd{\Child_{\variableIndex}}}

\newcommand{\PseudoChild}{\mathcmd{\mathrm{\bf{PC}}}}
\newcommand{\PseudoChildIndexed}{\mathcmd{\PseudoChild_{\variableIndex}}}

==> style/commands/commands_dpop.tex <==
\newcommand{\utilityMessage}{\mathcmd{\mathfrak{U}}}
\newcommand{\utilityMessageIndexed}{\mathcmd{\utilityMessage_\agentIndex^\agentIndexOther}}



\newcommand{\utilityMessageLongDomain}{\mathcmd{
  \utilityMessage ~:~ \realsSet^{|\domainSet_1|} \times \dots \times \realsSet^{|\domainSet_{\numberOfVariables}|} \rightarrow \realsSet
}}

\newcommand{\utilityVariable}{\mathcmd{\mathfrak{u}}}

\newcommand{\utilityMessageChildrenIndexed}{\mathcmd{\utilityMessage^\agentIndex_{\Child_{\agentIndex}}}}
\newcommand{\utilityMessageChildrenIndexedLong}{\mathcmd{
  \utilityMessageChildrenIndexed = \bigoplus_{\agent_\agentIndexOtherOther \in \Child_{\agentIndex}} \utilityMessage^\agentIndex_\agentIndexOtherOther
}}

\newcommand{\utilityMessageParentsIndexed}{\mathcmd{\utilityMessage^\agentIndexOther_{\Parent_{\agentIndex}}}}
\newcommand{\utilityMessageParentsIndexedLong}{\mathcmd{
  \utilityMessageParentsIndexed = \operator(\functionSetSharedIndexed)
}}

\newcommand{\utilityMessageLocalIndexed}{\mathcmd{\utilityMessage_\agentIndex}}
\newcommand{\utilityMessageLocalIndexedLong}{\mathcmd{
  \utilityMessageLocalIndexed = \operator(\functionSetLocalIndexed)
}}

\newcommand{\utilityMessageAgentIndexed}{\mathcmd{\utilityMessage^\agentIndex}}
\newcommand{\utilityMessageAgentLongIndexed}{\mathcmd{
  \utilityMessageAgentIndexed = \utilityMessageAgentLocalIndexed \join \utilityMessageChildrenIndexed \join \utilityMessageParentsIndexed
}}

\newcommand{\utilityMessageAgentLocalIndexed}{\mathcmd{\utilityMessage_\agentIndex}}


==> style/commands/commands_indexes.tex <==
\newcommand{\functionIndex}{\mathcmd{n}}
\newcommand{\functionIndexOther}{\mathcmd{p}}

\newcommand{\agentIndex}{\mathcmd{i}}  
\newcommand{\agentIndexOther}{\mathcmd{j}} 
\newcommand{\agentIndexOtherOther}{\mathcmd{k}} 

\newcommand{\agentIndexParent}{\mathcmd{j}} 
\newcommand{\agentIndexChild}{\mathcmd{k}} 
\newcommand{\agentIndexRoot}{\mathcmd{1}}

\newcommand{\variableIndex}{\mathcmd{i}}
\newcommand{\variableIndexOther}{\mathcmd{j}}

\newcommand{\observationIndex}{\mathcmd{s}}

\newcommand{\numberOfObservations}{\mathcmd{S}}
\newcommand{\numberOfAgents}{\mathcmd{M}}
\newcommand{\numberOfVariables}{\mathcmd{N}}
\newcommand{\numberOfFunctions}{\mathcmd{K}}

\newcommand{\realsSet}{\mathcmd{\mathds{R}}}
\newcommand{\naturalSet}{\mathcmd{\mathds{N}}}

\newcommand{\transpose}{\mathrm{T}}

==> style/commands/commands_proof.tex <==
\newcommand{\meanFunctionObservation}{\mathcmd{
    \meanFunctionBase_\observationIndex(\functionInputBase | \observationSet)
}}
\newcommand{\meanFunctionObservationDot}{\mathcmd{
    \meanFunctionBase_\observationIndex(\cdot | \observationSet)
}}

\newcommand{\varianceFunctionObservation}{\mathcmd{
    \varianceFunctionBase_\observationIndex(\functionInputBase | \observationSet)
}}

\newcommand{\varianceFunctionObservationDot}{\mathcmd{
    \varianceFunctionBase_\observationIndex(\cdot | \observationSet)
}}

\newcommand{\deviationFunctionObservation}{\mathcmd{
    \deviationFunctionBase_\observationIndex(\functionInputBase | \observationSet)
}}
\newcommand{\deviationFunctionObservationDot}{\mathcmd{
    \deviationFunctionBase_\observationIndex(\cdot | \observationSet)
}}

\newcommand{\upperBoundFunctionObservation}{\mathcmd{
    \upperBoundFunctionBase_{\observationIndex}(\functionInputBase | \observationSet)
}}
\newcommand{\upperBoundFunctionObservationDot}{\mathcmd{
    \upperBoundFunctionBase_{\observationIndex}(\cdot | \observationSet)
}}

\newcommand{\lipschitzConstantNormalized}{\mathcmd{
    \lipschitzConstantIndexed \functionInputObservationDelta
}}

\newcommand{\lipschitzConstantNormalizedLong}{\mathcmd{
    \lipschitzConstantNormalized = \lipschitzConstant \left( \functionInputObservation - \functionInputObservationLeft \right) = \lipschitzConstant \functionInputObservationDelta
}}

\newcommand{\functionOutputObservationConstantBase}{\mathcmd{
    \alpha_\observationIndex
}}
\newcommand{\functionOutputObservationConstant}{\mathcmd{
    \functionOutputObservationConstantBase(\observationSet)
}}

\newcommand{\functionOutputObservation}{\mathcmd{
    \functionOutputBase_{\observationIndex}
}}

\newcommand{\functionOutputObservationLeftLeft}{\mathcmd{
    \functionOutputBase_{\observationIndex - 2}
}}

\newcommand{\functionOutputObservationLeft}{\mathcmd{
    \functionOutputBase_{\observationIndex - 1}
}}

\newcommand{\functionOutputObservationRight}{\mathcmd{
    \functionOutputBase_{\observationIndex + 1}
}}

\newcommand{\functionOutputObservationRightRight}{\mathcmd{
    \functionOutputBase_{\observationIndex + 2}
}}

\newcommand{\functionInputObservation}{\mathcmd{
    \functionInputBase_{\observationIndex}
}}

\newcommand{\functionInputObservationLeftLeft}{\mathcmd{
    \functionInputBase_{\observationIndex-2}
}}

\newcommand{\functionInputObservationLeftLeftLeft}{\mathcmd{
    \functionInputBase_{\observationIndex-3}
}}

\newcommand{\functionInputObservationLeft}{\mathcmd{
    \functionInputBase_{\observationIndex-1}
}}

\newcommand{\functionInputObservationRight}{\mathcmd{
    \functionInputBase_{\observationIndex+1}
}}

\newcommand{\functionInputObservationRightRight}{\mathcmd{
    \functionInputBase_{\observationIndex+2}
}}

\newcommand{\functionInputObservationDelta}{\mathcmd{
    \Delta \functionInputBase_{\observationIndex}
}}

\newcommand{\functionInputObservationDeltaLong}{\mathcmd{
    \functionInputObservationDelta = \functionInputObservation - \functionInputObservationLeft
}}

\newcommand{\functionInputObservationNormalizedBase}{\mathcmd{
    \tau
}}

\newcommand{\functionInputObservationNormalized}{\mathcmd{
    \functionInputObservationNormalizedBase_{\observationIndex}(\functionInputBase | \observationSet)
}}

\newcommand{\functionInputObservationNormalizedLeft}{\mathcmd{
    \functionInputObservationNormalizedBase_{\observationIndex - 1}(\functionInputBase | \observationSet)
}}

\newcommand{\functionInputObservationNormalizedLong}{\mathcmd{
    \functionInputObservationNormalized =
    \frac{
        \functionInputBase - \functionInputObservationLeft
    }{
        \functionInputObservation - \functionInputObservationLeft
    }
}}

\newcommand{\functionInputObservationNormalizedCriticalPoint}{\mathcmd{
    \hat{\functionInputObservationNormalizedBase}_{\observationIndex}(\functionOutputObservationConstantBase|\observationSet)
}}

\newcommand{\functionInputObservationNormalizedCriticalPointLong}{\mathcmd{
    \functionInputObservationNormalizedCriticalPoint =
    \frac{1}{2}
    \left(
        \functionInputObservationNormalized + \functionInputObservationNormalizedLeft
    \right)
    +
    \frac{1}{2 \lipschitzConstantNormalized}
    \left(
        \functionOutputObservation - \functionOutputObservationLeft
    \right)
    =
    \frac{1}{2}
    \left(
        1 - \functionOutputObservationConstant
    \right)
}}

